Analytical bounds on the heat transport in internally heated convection

We obtain an analytical bound on the mean vertical convective heat flux $\langle w T \rangle$ between two parallel boundaries driven by uniform internal heating. We consider two configurations, one with both boundaries held at the same constant temperature, and the other one with a top boundary held at constant temperature and a perfectly insulating bottom boundary. For the first configuration, Arslan et al. (J. Fluid Mech. 919:A15, 2021) recently provided numerical evidence that Rayleigh-number-dependent corrections to the only known rigorous bound $\langle w T \rangle \leq 1/2$ may be provable if the classical background method is augmented with a minimum principle stating that the fluid's temperature is no smaller than that of the top boundary. Here, we confirm this fact rigorously for both configurations by proving bounds on $\langle wT \rangle$ that approach $1/2$ exponentially from below as the Rayleigh number is increased. The key to obtaining these bounds are inner boundary layers in the background fields with a particular inverse-power scaling, which can be controlled in the spectral constraint using Hardy and Rellich inequalities. These allow for qualitative improvements in the analysis not available to standard constructions.

==> gio-intro.tex <==
Convection driven by buoyancy is abundant in geophysical and astrophysical flows, from atmospheric convection driving ocean currents to solar convection transporting heat in stars. The prototypical setup for studying these flows is that of Rayleigh--B\'enard convection, where flow in a layer of fluid is driven by the temperature differential across the boundaries. In reality, convection in many natural or engineering situations is at least partially driven by an internal heating source. Examples include convection in the Earth's mantle due to radiogenic heat \citep{davies1992mantle, schubert2001mantle,mulyukova2020}, convection in radiative planet atmospheres \citep{seager2010exoplanet, pierrehumbert2010principles, guervilly2019turbulent}, and engineering flows where exothermic chemical or nuclear reactions drive the convection \citep{tran2009effective}. Gaining insights into these physical and practical scenarios requires a thorough understanding of internally heated (IH) convection, and yet studies in this direction are relatively few.

Following the early investigations by \cite{roberts1967convection} and \cite{tritton1975internally}, research into IH convection has recently gained renewed momentum through computational analysis \citep{goluskin2012convection, goluskin2015internally, goluskin2015penetrative} and experiments \citep{lepot2018radiative, bouillaut2019transition,limare2019convection,limare2021transient}. However, a comprehensive understanding of flows driven by internal heating is far from complete and the behaviour of such flows in the limiting regime of extreme heating remains unknown. 

Here, we probe this regime using rigorous upper bounding theory. Specifically, we bound the mean vertical convective heat flux in two configurations of IH convection, one where the fluid is bounded between horizontal plates held at the same temperature and one where the bottom plate is replaced by a perfect insulator. These two configurations, which we refer to as IH1 and IH3 following the terminology introduced by \cite{goluskin2016internally}, are illustrated schematically in panels (a) and (b) of figure~\ref{Flow configuration: IH1 and IH3 figures}. %In both cases, a minimum principle ensures that the temperature of the fluid cannot be larger than that of the isothermal top boundary.

\begin{figure}
    \centering
    \begin{tabular}{lc}
    \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[scale = 0.45]{Figures/IH1_30_sept.eps}
    \caption{}
    \end{subfigure} &
    \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[scale = 0.45]{Figures/IH3_30_sept.eps}
    \caption{}
    \end{subfigure}
    \end{tabular}
    \caption{The two configurations considered in this paper. (a) IH1: Isothermal boundaries, (b) IH3: Isothermal top boundary and insulating bottom boundary. In both configurations the heating is uniform, so the non-dimensional thermal source term is $H = 1$.  Dashed lines show the temperature profiles in the pure conduction state, while solid lines sketch the temporally- and horizontally-averaged temperature profiles in a typical turbulent state (also shown using the color plot).}
     \label{Flow configuration: IH1 and IH3 figures}
\end{figure}

The mean vertical convective heat flux $\langle wT \rangle$, where $w$ and $T$ are the nondimensional vertical velocity and temperature and angled brackets denote space-time averages, has a slightly different physical interpretation in the two configurations. For the IH1 case, $\langle w T \rangle$  is related to the asymmetry in the heat fluxes $\mathcal{F}_T$ and $\mathcal{F}_B$ through the top and the bottom boundaries. Specifically, space-time averaging the dimensionless transport equation for temperature (see~\eqref{e:heat-ns} in \S\ref{s:setup}) multiplied by the wall-normal coordinate $z$ yields
\begin{equation}
\mathcal{F}_T = \frac{1}{2} + \langle w T \rangle, \qquad \mathcal{F}_B = \frac{1}{2} - \langle w T \rangle.
\end{equation}
In the purely conductive state, the heat generated inside the domain leaves equally between the two boundaries, hence $\mathcal{F}_T = \mathcal{F}_B = 1/2$. In the convective state, instead, the asymmetry of buoyancy combines with the uniform heat source to create boundary layers with different characteristics near the top and bottom boundaries, as illustrated in figure~\ref{Flow configuration: IH1 and IH3 figures}(a). The bottom boundary layer is stably stratified, whereas the top boundary layer is unstably stratified. Convective heat transport ($\langle wT\rangle > 0$) makes the top boundary layer thinner than the bottom one, so in any convective state one has $\mathcal{F}_T > \mathcal{F}_B$. Since the boundary temperature is fixed and the fluid is internally heated, one also expects the boundary flux $\mathcal{F}_B$ to remain non-negative, meaning that heat can escape from the bottom boundary but not enter through it. This fact can be proved rigorously (\citealp[Appendix~A.1]{goluskin2012convection}; \citealp[Appendix~A]{arslan2021bounds}) and translates into the following upper bounds on the vertical heat transport \citep{goluskin2012convection}:
\begin{equation}
\langle w T \rangle \leq \frac{1}{2} \quad \text{in IH1}.
\label{Introduction: hypothesis IH1}
\end{equation}

For the IH3 configuration, instead, the mean vertical flux $\langle w T \rangle$ is related to the difference of the horizontally-averaged temperature between the top $\overline{T}_T$ and the bottom wall $\overline{T}_B$. Indeed, upon multiplying the dimensionless evolution equation for the temperature (see~\eqref{e:heat-ns} in \S\ref{s:setup}) with the wall-normal coordinate $z$ and space-time averaging one obtains
\begin{eqnarray}
\langle w T \rangle  = \overline{T}_T -\overline{T}_B + \frac12.
\end{eqnarray}
The isothermal boundary condition implies that the temperature $T_T$ at the top boundary is in fact constant, so $\overline{T}_T = T_T$, and we take it be zero without loss of generality in our nondimensionalization. Since the nondimensional internal heating rate is positive, one expects the mean bottom temperature $\overline{T}_B$ to be non-negative. As before, this fact can be proved rigorously and results in the upper bound \cite[Chapter~1]{goluskin2016internally}
\begin{equation}
\langle w T \rangle \leq \frac{1}{2}\quad \text{in IH3}.
\label{Introduction: hypothesis IH3}
\end{equation}

For the IH1 configuration, \cite{arslan2021bounds} recently proved that $\langle w T \rangle \leq 2^{-21/5}R^{1/5}$, where $R$ is a nondimensional parameter that measures the strength of the internal heating and may be interpreted as a Rayleigh number. This result, which is independent of the Prandtl number $\Pran$, fails to improve the uniform bound in~\eqref{Introduction: hypothesis IH1} for $R > 2^{16}=65536$. However, numerical evidence by the same authors suggests that an upper bound on  $\langle w T \rangle$ approaching $1/2$ from below monotonically as $R$ is increased may be provable when the background method by Doering \& Constantin \citep{PhysRevLett.69.1648,PhysRevE.49.4087,PhysRevE.53.5957,PhysRevE.51.3192} is augmented with a minimum principle stating that the fluid's temperature cannot be smaller than that the top boundary. Unfortunately, they also provided a rather tantalizing proof that such a bound cannot be obtained using typical analytical constructions. 

In this paper we overcome this barrier and show that $R$-dependent bounds on $\langle wT \rangle$ strictly smaller than $1/2$ can be obtained analytically not only in the IH1 case, but also for the IH3 configuration. Precisely, we prove that
\begin{subequations} \label{intro bounds}
\begin{align} 
\label{e:ih1-bound-intro}
&&&&\langle w T \rangle &\leq \frac{1}{2} -  c_1 R^{\frac{1}{5}} \exp \left(-c_2 R^{\frac{3}{5}}\right) &\text{in IH1,} &&&&\\
&&&&\langle w T \rangle &\leq \frac{1}{2} -  \frac{c_3}{R^{\frac{1}{5}}} \exp \left(-c_4 R^{\frac{3}{5}}\right) &\text{in IH3,}&&&&
\label{e:ih3-bound-intro}
\end{align} 
\end{subequations}
%
where $c_1, c_2, c_3$ and $c_4$ are constants (independent of both $R$ and $\Pran$). To establish these results, we formulate a bounding principle for $\langle wT \rangle$ using the auxiliary functional method \citep{chernyshenko2014polynomial, fantuzzi2016bounds, tobasco2018optimal, chernyshenko2017relationship}. Our implementation of the method is equivalent to an application of the background method when the latter is augmented with a minimum principle for the temperature field and, for the IH1 case, is the same as that in \cite{arslan2021bounds}. The novelty aspects in our arguments are the use of a background temperature field with a lower boundary layer growing as $z^{-1}$, motivated by the numerical results by \citet{arslan2021bounds}, and the application of Hardy inequalities (IH1) and Rellich inequalities (IH3). Such inequalities have already been employed to prove bounds on convective flows at infinite Prandtl number \citep{doering2006bounds,whitehead2011internal} but, to the best of our knowledge, their use at finite Prandtl number is new.

The rest of this work is organized as follows. We start by describing the problem setup in \S 2.  In \S 3, we apply the auxiliary function method formulate upper bounding principles for $\langle wT \rangle$ in both IH1 and IH3 configurations. We then prove the upper bound~\eqref{e:ih1-bound-intro} in \S 4 and the upper bound~\eqref{e:ih3-bound-intro} in \S 5. Finally, \S 6, discusses our method of proof, compares our results with available phenomenological theories, and offers concluding remarks.
